TacDiffusion: Force-domain Diffusion Policy for Precise Tactile Manipulation

Assembly is a crucial skill for robots in both modern manufacturing and service robotics. However, mastering transferable insertion skills that can handle a variety of high-precision assembly tasks remains a significant challenge. This paper presents a novel framework that utilizes diffusion models to generate 6D wrench for high-precision tactile robotic insertion tasks. It learns from demonstrations performed on a single task and achieves a zero-shot transfer success rate of 95.7% across various novel high-precision tasks. Our method effectively inherits the self-adaptability demonstrated by our previous work. In this framework, we address the frequency misalignment between the diffusion policy and the real-time control loop with a dynamic system-based filter, significantly improving the task success rate by 9.15%. Furthermore, we provide a practical guideline regarding the trade-off between diffusion models' inference ability and speed.

==> 1_introduction.tex <==
\section{Introduction}

In recent years, robot learning has emerged as a pivotal technology in the field of robot manipulation, offering the potential to enhance the capabilities of robots in performing complex manipulation tasks across a wide variety of conditions. Recent results in computer science and robotics have demonstrated that high-capacity models with a broad generalization can be obtained by collecting a large dataset of demonstrations of robot behaviors and training an expressive policy to extract the desirable behaviors with imitation learning \cite{walke2023bridgedata, brohan2022rt, vuong2023open, fang2024rh20t, khazatsky2024droid}. Despite significant advancements, traditional methods often fall short in matching the performance of model-based approaches or the demonstrated behaviors, particularly when considering execution efficiency. 


% Despite significant advances, traditional methods often struggle to achieve the model-based methods' or demonstrated behaviors' level performance (in perspective of execution efficancy), particularly when applied in real-time scenarios where computational efficiency is critical. In , the authors highlight the critical importance of high control frequency in robot performance by demonstrating the difference in performances when drawing circles on a table with robots controlled at varying frequencies. 

There is extensive literature on learning a high-performance policy, particularly in the following areas: (a) \textit{Control frequency}: High control frequency is crucial for enhancing robot performance \cite{franklin1994feedback, ogata2020modern, chen2023passivity}. Integrating a neural network with fast inference speed into the real-time control loop has proven successful in various scenarios \cite{miller1994real, yang2018biologically, yang2018robot}. However, these models are typically small with limited capacity to capture the underlying relationships in complex data, leading to poor generalization ability; (b) Action Domain: Some researchers design their action space based on the force controller instead of a naive position controller and demonstrate an enhanced interactive performance with the environment \cite{shi2021combining, yuan2022sim,zhang2023efficient}. Nevertheless, concerns remain regarding the continuity of actions and the inconsistency between the network's output frequency and the control frequency. (c) \textit{Parameterized robot learning}: This approach typically focuses on learning core parameters of a model-based method, ensuring the implementability of the resulting outputs \cite{da2012learning, johannsmeier2019framework, wu2023learning, 10610835}. Since these parameters are often tailored to specific tasks, fine-tuning becomes mandatory when applying them to novel tasks.

This paper addresses these challenges by proposing a novel imitation learning framework based on diffusion models, specifically designed to enhance both the performance and adaptability of robotic tasks in real-time environments. 


Our approach integrates a dynamic system-based filter to mitigate the conflict between model accuracy and inference speed, ensuring smooth and reliable task execution even under varying computational loads.

The contributions of this work are threefold:
The development of a diffusion model-based imitation learning framework tailored for real-time robotic applications.
A systemic guideline on choosing the proper to model size to trade-off between model's accuracy and inference speed to reach the optimal performance in the real world task. 


The introduction of a dynamic system-based filter that enhances the robustness of action generation during task execution.
Extensive empirical validation demonstrating the superior transferability and efficiency of our approach on both trained and novel tasks.



P5: gap in research (poor performance than the model based policy):\\
1. policy output frequency (trade-off model's ability and speed)\\
2. the logging frequency of the training dataset is less addressed 
3. action design (domain)

P6: describe the paper, in this paper we ...\\

P7: the contribution of this paper\\
1) a full-fledged framework for collecting real-time (1000 Hz) training data, robot learning with given data and execute the learned policy safely and reach model based methods level implementable behavior; superior performance and transfer ability for novel tasks\\
2) demonstrate the importance of action frequency to contact-rich manipulation; prove that the conflict between the model-size and action output frequency can be effectively relieved with our DS based filter
    3) 

systemic guideline
combine DF with torque controller


1. robot learning is fast developing, however, the performance of the trained policy on the real setup is normally not as good as the traditional model-based method (RL is not in our discussion scope)

2. The reasons are:
a. 
b. action space design (force domain comparing to position domain actions)
c. the data logging frequency of the original 

The reasons a and c are in a cyclical cause-and-effect relationship.

Fig: EE's displacement vs implementable continuous trajectory


related papers: 
\cite{pearce2022imitating} -- diffusion model we used \\
\cite{reuss2023goal, chi2023diffusion} -- related DF model application in manipulator, but in vision field \\

\cite{nakkiran2024step} -- guidance paper of diffusion model derivation \\
\cite{lin2024diffusion, yang2024survey} -- survey papers about diffusion model \\
